Mapping the Landscape of Independent Food Delivery Platforms in the United States

Beyond the well-known giants like Uber Eats and DoorDash, there are hundreds of independent food delivery platforms in the United States. However, little is known about the sociotechnical landscape of these ``indie'' platforms. In this paper, we analyzed these platforms to understand why they were created, how they operate, and what technologies they use. We collected data on 495 indie platforms and detailed survey responses from 29 platforms. We found that personalized, timely service is a central value of indie platforms, as is a sense of responsibility to the local community they serve. Indie platforms are motivated to provide fair rates for restaurants and couriers. These alternative business practices differentiate them from mainstream platforms. Though indie platforms have plans to expand, a lack of customizability in off-the-shelf software prevents independent platforms from personalizing services for their local communities. We show that these platforms are a widespread and longstanding fixture of the food delivery market. We illustrate the diversity of motivations and values to explain why a one-size-fits-all support is insufficient, and we discuss the siloing of technology that inhibits platforms' growth. Through these insights, we aim to promote future HCI research into the potential development of public-interest technologies for local food delivery.

==> sections/7_conclusion.tex <==
\section{Conclusion}
Indie platforms have been a relatively unexplored player in the food delivery landscape. In this work, we aimed to start mapping the hundreds of indie food delivery platforms across the United States and to investigate why and how they operate. We found that many of these platforms have been in operation for several years, and continue to grow through location expansions, customer acquisition, and restaurant partnerships. Indie platforms are committed to their vision of ``being local,'' which may look like collaborations with under-served independent restaurants, donating to charities, and hiring local couriers to keep profits within their community. We found that indie platforms adapt their services to provide timely, personalized service to their stakeholders, such as through phone ordering and easily accessible live customer support. Cost constraints many platforms to off-the-shelf solutions, which lack the customizability for platforms to agilely respond to stakeholders' needs. 

Our study presented three implications for future research and investigation. We showed that indie platforms are a widespread fixture of the food delivery landscape, that the diversity in their motivations, needs, and values makes one size fits all solutions inadequate, and that the silos created by the off-the-shelf solution impede their operations. Our survey revealed that being local allows indie platforms to not only provide improved quality and speed of service, but potentially better rates than mainstream platforms. Indie platforms are in a period of transition as they plan to grow and expand, and are in need of flexible software that can meet their evolving needs. 
